A Bramble-Pasciak conjugate gradient method for discrete Stokes equations with random viscosity

We study the iterative solution of linear systems of equations arising from stochastic Galerkin finite element discretizations of saddle point problems. We focus on the Stokes model with random data parametrized by uniformly distributed random variables and discuss well-posedness of the variational formulations. We introduce a Bramble-Pasciak conjugate gradient method as a linear solver. It builds on a non-standard inner product associated with a block triangular preconditioner. The block triangular structure enables more sophisticated preconditioners than the block diagonal structure usually applied in MINRES methods. We show how the existence requirements of a conjugate gradient method can be met in our setting. We analyze the performance of the solvers depending on relevant physical and numerical parameters by means of eigenvalue estimates. For this purpose, we derive bounds for the eigenvalues of the relevant preconditioned sub-matrices. We illustrate our findings using the flow in a driven cavity as a numerical test case, where the viscosity is given by a truncated Karhunen-Lo\`eve expansion of a random field. In this example, a Bramble-Pasciak conjugate gradient method with block triangular preconditioner outperforms a MINRES method with block diagonal preconditioner in terms of iteration numbers.

==> ea_block_diag.tex <==
\subsection{The block diagonal preconditioned SGFE problem}
\label{subsec_block_diag}
For bounds on the eigenvalues of the block diagonal preconditioned SGFE problem, we use a result from  
\cite{ErnstEtAl2009} and adjust it to the prevailing setting.
\begin{theorem}[Theorem 4.1 in \cite{ErnstEtAl2009}]
\label{theorem_block_diagonal_precon_ev}
Assume \cref{eq_ev_bounds_SGFE_diff_approx_diff} and \cref{eq_bounds_SGFE_quasi_Schur_approx_Schur} hold. 
Then, the eigenvalues of the block diagonal preconditioned matrix $\mathcal{P}_1^{-1} \mathcal{C}$, with 
$\mathcal{C}$ and $\mathcal{P}_1$ according to \cref{eq_block_matrix_form} and \cref{eq_block_precon}, 
respectively, lie in the union of the intervals $[-a,-b] \cup [c,d]$, where 
\begin{align}
\label{eq_ev_blk_diag_1}
a = \frac{\sqrt{\hat{\delta}^2 + 4\hat{\Theta}} - \hat{\delta}}{2}, \quad
b = \frac{\sqrt{\hat{\Delta}^2 + 4\hat{\theta}} - \hat{\Delta}}{2}, \quad
c = \hat{\delta}, \quad
d = \frac{\hat{\Delta} + \sqrt{\hat{\Delta}^2 + 4\hat{\Theta}}}{2}. 
\end{align}
\end{theorem}
\begin{proof}
See proof of \cite[Theorem 4.1]{ErnstEtAl2009}.
\end{proof}

==> ea_block_tri.tex <==
\subsection{\deleted[id=A]{The block triangular preconditioned SGFE problem}}
\label{subsec_block_tri}
\deleted[id=A]{We do not immediately restate the result for the eigenvalues of the triangular preconditioned matrix. First, we discuss the effect of using a negative sign for the Schur complement approximation and the scaling factor $a$ in $\mathcal{P}_2$ introduced in \cref{eq_block_precon}. In order to do this, we specify the scaling $a:= a_\delta \hat{\delta}$, with $0 < a_\delta < 1$ and $\hat{\delta}$ as in \mbox{\cref{lemma_eigenvalues_precon_diff}}, and define}
{\textcolor{red}{
\begin{align}
\cancel{\label{eq_inner_product_matrix}
\mathcal{H} := \begin{bmatrix} \mathcal{A} - a_{\delta} \hat{\delta}\widetilde{\mathcal{A}}_{\text{mg}} & 0 \\ 0 & 
\widetilde{\mathcal{S}}_p \end{bmatrix},}
\end{align}}}
\deleted[id=A]{with $\widetilde{\mathcal{A}}_{\text{mg}}$ and $\widetilde{\mathcal{S}}_p$ according to 
\cref{eq_block_precon}.}
\begin{lemma}
\label{lemma_ipcg_conditions}
\deleted[id=A]{Let $a$ in \cref{eq_block_precon} be set to $a= a_\delta \hat{\delta}$, with 
$0 < a_\delta < 1$ and $\hat{\delta}$ as in \mbox{\cref{lemma_eigenvalues_precon_diff}}. Then, the matrix $\mathcal{H}$ in
\cref{eq_inner_product_matrix} defines an inner product. Moreover, the triangular preconditioned system 
matrix $\mathcal{P}_2^{-1} \mathcal{C}$, with $\mathcal{C}$ and $\mathcal{P}_2$ according to 
\mbox{\cref{eq_block_matrix_form,eq_block_precon}}, respectively, is $\mathcal{H}$-symmetric and $\mathcal{H}$-positive definite, 
i.e.}
{\textcolor{red}{
\begin{align}
\label{eq_inner_product_cond_2a}
\hspace{2cm} &\mathcal{H} \mathcal{P}_2^{-1} \mathcal{C} = (\mathcal{P}_2^{-1}\mathcal{C})^T\mathcal{H}, \\[-4ex]\cline{1-2}
\label{eq_inner_product_cond_1a}
&\vecg{w}^{\text{T}} \mathcal{H} \mathcal{P}_2^{-1} \mathcal{C} \vecg{w} > 0, \hspace{2cm} \forall 
\vecg{w} \in \RR^{\nPC \nFE} \backslash\{\vecg{0}\}.\\[-4ex]\cline{1-2} \notag
\end{align}}}
\end{lemma}
\begin{proof}
\deleted[id=A]{First of all, we make sure that the matrix $\mathcal{H}$ defines an inner product, i.e.\ check that it is 
symmetric and positive definite. Subsequently, we establish  \cref{eq_inner_product_cond_2a} and \cref{eq_inner_product_cond_1a}.}

\deleted[id=A]{The symmetry of $\mathcal{H}$ is verified by noting that the building blocks of 
the matrices on the diagonal are symmetric. To verify positive definiteness of $\mathcal{H}$, we consider its diagonal blocks separately. The lower diagonal block $\widetilde{\mathcal{S}}_p = I \otimes D_P$ is positive definite because its 
Kronecker factors are positive definite, see \mbox{\cite[Section 3.5]{ElmanEtAl2014}}. The investigation of the upper diagonal 
block is more intricate: The matrix $\mathcal{A} - a_{\delta} \hat{\delta}\widetilde{\mathcal{A}}_{\text{mg}}$ is 
positive definite if}
{\textcolor{red}{
\begin{equation}
\cancel{\label{eq_condition_pd_upper}
\frac{\vecg{v}^{\text{T}}(\mathcal{A} - a_{\delta} \hat{\delta}\widetilde{\mathcal{A}}_{\text{mg}})
\vecg{v}}{\vecg{v}^{\text{T}} \vecg{v}} = \frac{\vecg{v}^{\text{T}}\mathcal{A} \vecg{v}}{\vecg{v}^{\text{T}} \vecg{v}}
 - \frac{\vecg{v}^{\text{T}}a_{\delta} \hat{\delta} \widetilde{\mathcal{A}}_{\text{mg}} \vecg{v}}{\vecg{v}^{\text{T}} \vecg{v}}
 >  0 \quad \forall \vecg{v} \in \RR^{\nPC \nFE_u} \backslash \{\vecg{0}\}. }
\end{equation}}}
\deleted[id=A]{We can express this condition equivalently by rearranging \cref{eq_condition_pd_upper}:}
{\textcolor{red}{
\begin{equation}
\cancel{\label{eq_condition_pd_bpcg}
\min_{\vecg{v}\in \RR^{\nPC \nFE_u} \backslash \{\vecg{0}\}} 
\frac{\vecg{v}^{\text{T}}\mathcal{A} \vecg{v}}{\vecg{v}^{\text{T}} a_{\delta} \hat{\delta}\widetilde{\mathcal{A}}_{\text{mg}}
\vecg{v}} > 1.}
\end{equation}}}
\deleted[id=A]{From \cref{eq_ev_bounds_SGFE_diff_approx_diff} and $0 < a_\delta < 1$, we can deduce $\lambda_{\text{min}}(a_{\delta}^{-1} \hat{\delta}^{-1} \widetilde{\mathcal{A}}_{\text{mg}}^{-1} \mathcal{A}) \geq 
a_\delta^{-1} > 1$, which eventually ensures the positive definiteness of 
$\mathcal{A} - a_{\delta} \hat{\delta}\widetilde{\mathcal{A}}_{\text{mg}}$ and thereby the positive 
definiteness of $\mathcal{H}$.}

\deleted[id=A]{In order to see that \cref{eq_inner_product_cond_2a} holds, we perform the matrix-matrix products on 
both sides of the equals sign and ascertain that the results are identical.~Establishing 
\cref{eq_inner_product_cond_1a} works exactly as in the case with deterministic data, using a matrix 
factorization in the form of a congruence transform, see \mbox{\cite[Lemma 3.3]{Klawonn1998}}.}
\end{proof}
\deleted[id=A]{In their 1988 paper \mbox{\cite{BramblePasciak1988}}, Bramble and Pasciak discovered the matrix $\mathcal{H}$ 
and its extraordinary effect on a triangular preconditioned problem structurally equivalent to 
$\mathcal{P}_2^{-1} \mathcal{C}$: The properties verified in \mbox{\cref{lemma_ipcg_conditions}} imply the existence 
of a CG method in the $\mathcal{H} \mathcal{P}_2^{-1} \mathcal{C}$-inner product \mbox{\cite{FaberManteuffel1984}}. 
Consequently, we can use the Bramble-Pasciak conjugate gradient (BPCG) method introduced in 
\mbox{\cite{BramblePasciak1988}} also to solve the SGFE problem considered in this work.}

\deleted[id=A]{To formulate the following theorem, we state a rescaled version of \cref{eq_ev_bounds_SGFE_diff_approx_diff}:}
{\textcolor{red}{
\begin{align}
\cancel{\label{eq_ev_bounds_SGFE_diff_approx_diff_scaled}
1 < a_{\delta}^{-1}  \leq \frac{\vecg{v}^{\text{T}}\mathcal{A}\vecg{v}}
{\vecg{v}^{\text{T}} \, a_{\delta} \hat{\delta} \widetilde{\mathcal{A}}_{\text{mg}} \vecg{v}} 
\leq a_{\delta}^{-1} \frac{\hat{\Delta}}{\hat{\delta}}, 
\quad \forall \vecg{v} \in \RR^{\nPC \nFE_u} \backslash \{\vecg{0}\},}
\end{align}}}
\deleted[id=A]{with $0<a_\delta < 1$ and $\hat{\delta}$, $\hat{\Delta}$ as in 
\mbox{\cref{lemma_eigenvalues_precon_diff}}. Now, we can use a result from \mbox{\cite{Zulehner2001}}.} 
\begin{theorem}[{\deleted[id=A]{Theorem 4.1 in \mbox{\cite{Zulehner2001}}}}]
\label{theorem_ev_bounds_zulehner}
\deleted[id=A]{Assume that \mbox{\cref{eq_ev_bounds_SGFE_Schur_approx_Schur,eq_ev_bounds_SGFE_diff_approx_diff_scaled}}
hold and let the matrices $\mathcal{C}$ and $\mathcal{P}_2$ be defined according to \cref{eq_block_matrix_form} and \cref{eq_block_precon} with $a= a_\delta \hat{\delta}$, $0 < a_\delta < 1$ and $\hat{\delta}$ as defined in \mbox{\cref{lemma_eigenvalues_precon_diff}}.~Then, the eigenvalues of the triangular preconditioned matrix $\mathcal{P}_2^{-1}\mathcal{C}$ lie in the interval $[1-\zeta_2,1-\zeta_1]$, where }
{\textcolor{red}{
\begin{align}
\label{eq_block_tri_ev_lower}
\zeta_1 &= \frac{2-(1+\hat{\Gamma})a_\delta^{-1} \frac{\hat{\Delta}}{\hat{\delta}}}{2}
-\sqrt{\frac{\Big(2-(1+\hat{\Gamma})a_\delta^{-1} \frac{\hat{\Delta}}{\hat{\delta}}\Big)^2}{4} + 
a_\delta^{-1} \frac{\hat{\Delta}}{\hat{\delta}} -1}, \\[-4ex]\cline{1-2} 
\label{eq_block_tri_ev_upper}
\zeta_2 &= \frac{2-(1+\hat{\gamma})a_\delta^{-1} \frac{\hat{\Delta}}{\hat{\delta}}}{2}
+ \sqrt{\frac{\Big(2-(1+\hat{\gamma})a_\delta^{-1} \frac{\hat{\Delta}}{\hat{\delta}}\Big)^2}{4} + 
a_\delta^{-1} \frac{\hat{\Delta}}{\hat{\delta}} -1}.\\[-4ex]\cline{1-2} \notag
\end{align}}}
\end{theorem}
\begin{proof}
\deleted[id=A]{See proof of \mbox{\cite[Theorem 4.1]{Zulehner2001}.}}
\end{proof}
% The construction of the block triangular preconditioner does not imply a particular relation between 
% $\widetilde{G}_S$ and $\widetilde{G}_A$. This is different to the block diagonal case in 
% \cref{subsec_precon_pseudo_Schur}, which suggested $\widetilde{G}_S = \widetilde{G}_A^{-1}$. Still, from our 
% numerical results (see \cref{figure_variation_k_s}) we can deduce that this choice is also reasonable in 
% the context of block triangular preconditioning using the KPP.
% Having a closer look at the eigenvalue bounds in Theorem \cref{theorem_ev_bounds_zulehner} reveals that the 
% choosing $\widetilde{G}_S = \widetilde{G}_A^{-1}$ might also be beneficial in this case. When we insert the 
% detailed versions \cref{eq_ev_bounds_SGFE_delta_hat}, \cref{eq_ev_bounds_SGFE_Delta_hat}, 
% \cref{eq_ev_bounds_SGFE_gamma_hat} and \cref{eq_ev_bounds_SGFE_Gamma_hat} into the relevant term, we get
% \begin{align}
% \hat{\Gamma} a_\delta^{-1} \frac{\hat{\Delta}}{\hat{\delta}} &= a_\delta^{-1} 
% \frac{(1+\sqrt{3} \, \chi)\, \Delta \, \overline{\nu}_0 \, \Theta^2 \, \overline{g}_A}
% {(1-\sqrt{3}\chi)^2\, \delta \,\underline{\nu}_0^2 \, \underline{g}_S  \, \underline{g}_A} = 
% a_\delta^{-1} \frac{(1+\sqrt{3} \, \chi)\, \Delta \, \overline{\nu}_0 \, \Theta^2}
% {(1-\sqrt{3}\chi)^2 \, \delta\, \underline{\nu}_0^2} \frac{ \overline{g}_A}{\underline{g}_S \, \underline{g}_A}, \\
% \hat{\gamma} a_\delta^{-1} \frac{\hat{\Delta}}{\hat{\delta}} &= a_\delta^{-1} 
% \frac{(1+\sqrt{3} \, \chi)  \, \Delta \, \overline{\nu}_0 \, \theta^2 \gamma^2 \, \overline{g}_A}
% {(1+\sqrt{3}\chi)(1-\sqrt{3} \, \chi) \, \delta\, \underline{\nu}_0\, \overline{\nu}_0 \, \overline{g}_S  \, \underline{g}_A} 
% = \frac{\Delta \, \theta^2 \gamma^2}
% {(1-\sqrt{3} \, \chi) \, \delta\, \underline{\nu}_0} 
% \frac{\overline{g}_A}{\overline{g}_S  \, \underline{g}_A}.
% \end{align}
% With respect to The choice $\widetilde{G}_S = \widetilde{G}_A^{-1}$ 
